MAD: Modality-Adaptive Decoding for Mitigating Cross-Modal Hallucinations in Multimodal Large Language Models

Multimodal Large Language Models (MLLMs) suffer from cross-modal hallucinations, where one modality inappropriately influences generation about another, leading to fabricated output. This exposes a more fundamental deficiency in modality-interaction control. To address this, we propose Modality-Adaptive Decoding (MAD), a training-free method that adaptively weights modality-specific decoding branches based on task requirements. MAD leverages the model's inherent ability to self-assess modality relevance by querying which modalities are needed for each task. The extracted modality probabilities are then used to adaptively weight contrastive decoding branches, enabling the model to focus on relevant information while suppressing cross-modal interference. Extensive experiments on CMM and AVHBench demonstrate that MAD significantly reduces cross-modal hallucinations across multiple audio-visual language models (7.8\% and 2.0\% improvements for VideoLLaMA2-AV, 8.7\% and 4.7\% improvements for Qwen2.5-Omni). Our approach demonstrates that explicit modality awareness through self-assessment is crucial for robust multimodal reasoning, offering a principled extension to existing contrastive decoding methods. Our code is available at \href{https://github.com/top-yun/MAD}{https://github.com/top-yun/MAD}

==> tables/tabel_cmm.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{0.9}
\renewcommand{\tabcolsep}{2.0mm}
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & 
\multicolumn{2}{c}{\textbf{Visual Dom.}} & 
\multicolumn{2}{c}{\textbf{Audio Dom.}} & 
\multicolumn{2}{c}{\textbf{Language Dom.}} &
\multirow{2}{*}{\textbf{Overall Acc. (\%)}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
 & \textbf{pa$\uparrow$} & \textbf{hr$\uparrow$} 
 & \textbf{pa$\uparrow$} & \textbf{hr$\uparrow$}
 & \textbf{pa$\uparrow$} & \textbf{hr$\uparrow$} &  \\
\midrule
VideoLLaMA2-AV             & 89.0 & 57.0 & 91.5 & 76.0 & 84.0 & 60.0 & 76.3 \\
VideoLLaMA2-AV + VCD       & 84.5 & 58.0 & 91.0 & 75.5 & 83.5 & 66.0 & 76.4 \\
VideoLLaMA2-AV + AVCD      & 88.0 & 55.5 & 92.5 & 75.5 & 84.0 & 59.0 & 75.8 \\
VideoLLaMA2-AV + MAD       & 87.0 & 77.5 & 92.5 & 76.0 & 84.0 & 71.0 & 81.3 \\
\midrule
video-SALMONN-7B          & 77.0 & 55.0 & 96.5 & 45.5 & 84.5 & 16.5 & 62.5 \\
video-SALMONN-7B + VCD     & 79.5 & 56.5 & 93.0 & 49.0 & 81.5 & 20.0 & - \\
video-SALMONN-7B + AVCD    & 72.5 & 63.0 & 96.0 & 43.0 & 85.0 & 21.5 & 63.5 \\
video-SALMONN-7B + MAD     & 69.5 & 73.5 & 96.0 & 49.5 & 90.0 & 23.5 & 67.0 \\
\midrule
Qwen2.5-Omni-7B            & 98.0 & 31.0 & 93.5 & 51.0 & 82.0 & 80.5 & 72.7 \\
Qwen2.5-Omni-7B + VCD      & 98.5 & 26.5 & 92.5 & 50.0 & 85.5 & 83.5 & - \\
Qwen2.5-Omni-7B + AVCD     & - & - & - & - & - & - & - \\
Qwen2.5-Omni-7B + MAD      & 97.0 & 56.5 & 88.5 & 80.0 & 81.5 & 85.5 & 81.5 \\
\bottomrule
\end{tabular}
\label{tab:cmm_results}
\end{table*}

